The Geography of Facebook Groups in the United States

We use exploratory factor analysis to investigate the online persistence of known community-level patterns of social capital variance in the U.S. context. Our analysis focuses on Facebook groups, specifically those that tend to connect users in the same local area. We investigate the relationship between established, localized measures of social capital at the county level and patterns of participation in Facebook groups in the same areas. We identify four main factors that distinguish Facebook group engagement by county. The first captures small, private groups, dense with friendship connections. The second captures very local and small groups. The third captures non-local, large, public groups, with more age mixing. The fourth captures partially local groups of medium to large size. The first and third factor correlate with community level social capital measures, while the second and fourth do not. Together and individually, the factors are predictive of offline social capital measures, even controlling for various demographic attributes of the counties. Our analysis reveals striking patterns of correlation between established measures of social capital and patterns of online interaction in local Facebook groups. To our knowledge this is the first systematic test of the association between offline regional social capital and patterns of online community engagement in the same regions.

==> figures/grand_summary_table.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Fri, Oct 08, 2021 - 02:59:20 PM
\begin{table}[!htbp] \centering 
  \caption{} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Statistic & \multicolumn{1}{c}{N} & \multicolumn{1}{c}{Mean} & \multicolumn{1}{c}{St. Dev.} & \multicolumn{1}{c}{Min} & \multicolumn{1}{c}{Pctl(25)} & \multicolumn{1}{c}{Pctl(75)} & \multicolumn{1}{c}{Max} \\ 
\hline \\[-1.8ex] 
\hline \\[-1.8ex] 
\end{tabular} 
\end{table} 


==> figures/local_cormat.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Thu, Oct 07, 2021 - 12:05:40 PM
\begin{tabular}{@{\extracolsep{5pt}} ccccccccccccccccccccccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Community health & percent\_black & premature\_mortality\_rate & mean\_commute\_time & non\_religious\_non\_profit\_organizations\_p\_1\_000 & religious\_congregations\_p\_1\_000 & Population & Density & institutional\_health & -violent\_crimes\_p\_100\_000 & \% Rural & Median HH income & Debt in collection & Poverty rate & Relative immobility & Income inequality & Premature Mortality & Disconnected youth & \% adults without BA & \% Black & \% White & \% Hispanic & Ethnic fractionalization & Black/white segration & community.health.controlled & num\_users\_per\_map \\ 
\hline \\[-1.8ex] 
Community health & $1$ & $$-$0.562$ & $$-$0.241$ & $$-$0.234$ & $0.838$ & $0.526$ & $$-$0.577$ & $$-$0.612$ & $0.423$ & $0.383$ & $0.398$ & $0.061$ & $$-$0.536$ & $$-$0.291$ & $$-$0.279$ & $$-$0.203$ & $$-$0.241$ & $$-$0.340$ & $$-$0.108$ & $$-$0.562$ & $0.384$ & $$-$0.215$ & $$-$0.388$ & $$-$0.284$ & $0.719$ & $0.040$ \\ 
percent\_black & $$-$0.562$ & $1$ & $0.300$ & $0.141$ & $$-$0.499$ & $$-$0.232$ & $0.418$ & $0.497$ & $$-$0.230$ & $$-$0.460$ & $$-$0.335$ & $$-$0.157$ & $0.530$ & $0.346$ & $0.550$ & $0.340$ & $0.300$ & $0.258$ & $0.041$ & $1$ & $$-$0.609$ & $0.122$ & $0.644$ & $0.302$ & $$-$0.339$ & $$-$0.311$ \\ 
premature\_mortality\_rate & $$-$0.241$ & $0.300$ & $1$ & $0.179$ & $$-$0.400$ & $0.411$ & $$-$0.195$ & $$-$0.120$ & $$-$0.509$ & $$-$0.298$ & $0.237$ & $$-$0.717$ & $0.741$ & $0.685$ & $0.516$ & $0.330$ & $1$ & $0.445$ & $0.633$ & $0.300$ & $$-$0.185$ & $$-$0.197$ & $0.149$ & $0.133$ & $$-$0.419$ & $$-$0.047$ \\ 
mean\_commute\_time & $$-$0.234$ & $0.141$ & $0.179$ & $1$ & $$-$0.273$ & $0.019$ & $$-$0.020$ & $0.039$ & $$-$0.182$ & $0.019$ & $0.227$ & $$-$0.108$ & $0.245$ & $0.126$ & $0.066$ & $0.014$ & $0.179$ & $0.095$ & $0.286$ & $0.141$ & $$-$0.011$ & $$-$0.088$ & $0.009$ & $$-$0.009$ & $$-$0.294$ & $$-$0.027$ \\ 
non\_religious\_non\_profit\_organizations\_p\_1\_000 & $0.838$ & $$-$0.499$ & $$-$0.400$ & $$-$0.273$ & $1$ & $0.236$ & $$-$0.351$ & $$-$0.394$ & $0.399$ & $0.289$ & $0.168$ & $0.230$ & $$-$0.588$ & $$-$0.396$ & $$-$0.308$ & $$-$0.144$ & $$-$0.400$ & $$-$0.344$ & $$-$0.337$ & $$-$0.499$ & $0.355$ & $$-$0.091$ & $$-$0.336$ & $$-$0.192$ & $0.730$ & $0.073$ \\ 
religious\_congregations\_p\_1\_000 & $0.526$ & $$-$0.232$ & $0.411$ & $0.019$ & $0.236$ & $1$ & $$-$0.793$ & $$-$0.716$ & $$-$0.075$ & $0.220$ & $0.697$ & $$-$0.478$ & $0.146$ & $0.215$ & $0.176$ & $0.040$ & $0.411$ & $0.188$ & $0.486$ & $$-$0.232$ & $0.199$ & $$-$0.307$ & $$-$0.232$ & $$-$0.192$ & $0.066$ & $$-$0.094$ \\ 
Population & $$-$0.577$ & $0.418$ & $$-$0.195$ & $$-$0.020$ & $$-$0.351$ & $$-$0.793$ & $1$ & $0.875$ & $$-$0.011$ & $$-$0.370$ & $$-$0.755$ & $0.311$ & $0.029$ & $$-$0.038$ & $0.049$ & $0.099$ & $$-$0.195$ & $0.067$ & $$-$0.414$ & $0.418$ & $$-$0.247$ & $0.259$ & $0.302$ & $0.341$ & $0.034$ & $0.119$ \\ 
Density & $$-$0.612$ & $0.497$ & $$-$0.120$ & $0.039$ & $$-$0.394$ & $$-$0.716$ & $0.875$ & $1$ & $0.047$ & $$-$0.289$ & $$-$0.656$ & $0.269$ & $0.081$ & $$-$0.031$ & $0.190$ & $0.100$ & $$-$0.120$ & $$-$0.067$ & $$-$0.347$ & $0.497$ & $$-$0.156$ & $0.115$ & $0.217$ & $0.345$ & $$-$0.026$ & $0.005$ \\ 
institutional\_health & $0.423$ & $$-$0.230$ & $$-$0.509$ & $$-$0.182$ & $0.399$ & $$-$0.075$ & $$-$0.011$ & $0.047$ & $1$ & $0.308$ & $0.006$ & $0.447$ & $$-$0.638$ & $$-$0.551$ & $$-$0.221$ & $$-$0.298$ & $$-$0.509$ & $$-$0.421$ & $$-$0.402$ & $$-$0.230$ & $0.349$ & $$-$0.185$ & $$-$0.321$ & $$-$0.139$ & $0.536$ & $$-$0.036$ \\ 
-violent\_crimes\_p\_100\_000 & $0.383$ & $$-$0.460$ & $$-$0.298$ & $0.019$ & $0.289$ & $0.220$ & $$-$0.370$ & $$-$0.289$ & $0.308$ & $1$ & $0.399$ & $0.183$ & $$-$0.448$ & $$-$0.357$ & $$-$0.299$ & $$-$0.313$ & $$-$0.298$ & $$-$0.413$ & $$-$0.021$ & $$-$0.460$ & $0.500$ & $$-$0.259$ & $$-$0.505$ & $$-$0.224$ & $0.243$ & $0.113$ \\ 
\% Rural & $0.398$ & $$-$0.335$ & $0.237$ & $0.227$ & $0.168$ & $0.697$ & $$-$0.755$ & $$-$0.656$ & $0.006$ & $0.399$ & $1$ & $$-$0.339$ & $0.013$ & $0.081$ & $0.040$ & $$-$0.099$ & $0.237$ & $$-$0.051$ & $0.460$ & $$-$0.335$ & $0.372$ & $$-$0.420$ & $$-$0.397$ & $$-$0.264$ & $$-$0.050$ & $$-$0.043$ \\ 
Median HH income & $0.061$ & $$-$0.157$ & $$-$0.717$ & $$-$0.108$ & $0.230$ & $$-$0.478$ & $0.311$ & $0.269$ & $0.447$ & $0.183$ & $$-$0.339$ & $1$ & $$-$0.589$ & $$-$0.829$ & $$-$0.395$ & $$-$0.425$ & $$-$0.717$ & $$-$0.362$ & $$-$0.650$ & $$-$0.157$ & $0.097$ & $0.230$ & $$-$0.032$ & $$-$0.085$ & $0.274$ & $0.195$ \\ 
Debt in collection & $$-$0.536$ & $0.530$ & $0.741$ & $0.245$ & $$-$0.588$ & $0.146$ & $0.029$ & $0.081$ & $$-$0.638$ & $$-$0.448$ & $0.013$ & $$-$0.589$ & $1$ & $0.697$ & $0.524$ & $0.409$ & $0.741$ & $0.574$ & $0.522$ & $0.530$ & $$-$0.483$ & $0.090$ & $0.434$ & $0.186$ & $$-$0.626$ & $$-$0.167$ \\ 
Poverty rate & $$-$0.291$ & $0.346$ & $0.685$ & $0.126$ & $$-$0.396$ & $0.215$ & $$-$0.038$ & $$-$0.031$ & $$-$0.551$ & $$-$0.357$ & $0.081$ & $$-$0.829$ & $0.697$ & $1$ & $0.439$ & $0.548$ & $0.685$ & $0.361$ & $0.522$ & $0.346$ & $$-$0.350$ & $$-$0.052$ & $0.292$ & $0.200$ & $$-$0.383$ & $$-$0.230$ \\ 
Relative immobility & $$-$0.279$ & $0.550$ & $0.516$ & $0.066$ & $$-$0.308$ & $0.176$ & $0.049$ & $0.190$ & $$-$0.221$ & $$-$0.299$ & $0.040$ & $$-$0.395$ & $0.524$ & $0.439$ & $1$ & $0.310$ & $0.516$ & $0.091$ & $0.275$ & $0.550$ & $$-$0.261$ & $$-$0.176$ & $0.267$ & $0.276$ & $$-$0.253$ & $$-$0.201$ \\ 
Income inequality & $$-$0.203$ & $0.340$ & $0.330$ & $0.014$ & $$-$0.144$ & $0.040$ & $0.099$ & $0.100$ & $$-$0.298$ & $$-$0.313$ & $$-$0.099$ & $$-$0.425$ & $0.409$ & $0.548$ & $0.310$ & $1$ & $0.330$ & $0.076$ & $0.037$ & $0.340$ & $$-$0.353$ & $0.048$ & $0.318$ & $0.188$ & $$-$0.179$ & $$-$0.310$ \\ 
Premature Mortality & $$-$0.241$ & $0.300$ & $1$ & $0.179$ & $$-$0.400$ & $0.411$ & $$-$0.195$ & $$-$0.120$ & $$-$0.509$ & $$-$0.298$ & $0.237$ & $$-$0.717$ & $0.741$ & $0.685$ & $0.516$ & $0.330$ & $1$ & $0.445$ & $0.633$ & $0.300$ & $$-$0.185$ & $$-$0.197$ & $0.149$ & $0.133$ & $$-$0.419$ & $$-$0.047$ \\ 
Disconnected youth & $$-$0.340$ & $0.258$ & $0.445$ & $0.095$ & $$-$0.344$ & $0.188$ & $0.067$ & $$-$0.067$ & $$-$0.421$ & $$-$0.413$ & $$-$0.051$ & $$-$0.362$ & $0.574$ & $0.361$ & $0.091$ & $0.076$ & $0.445$ & $1$ & $0.527$ & $0.258$ & $$-$0.459$ & $0.339$ & $0.379$ & $0.220$ & $$-$0.364$ & $$-$0.103$ \\ 
\% adults without BA & $$-$0.108$ & $0.041$ & $0.633$ & $0.286$ & $$-$0.337$ & $0.486$ & $$-$0.414$ & $$-$0.347$ & $$-$0.402$ & $$-$0.021$ & $0.460$ & $$-$0.650$ & $0.522$ & $0.522$ & $0.275$ & $0.037$ & $0.633$ & $0.527$ & $1$ & $0.041$ & $0.023$ & $$-$0.221$ & $$-$0.082$ & $0.081$ & $$-$0.392$ & $$-$0.060$ \\ 
\% Black & $$-$0.562$ & $1$ & $0.300$ & $0.141$ & $$-$0.499$ & $$-$0.232$ & $0.418$ & $0.497$ & $$-$0.230$ & $$-$0.460$ & $$-$0.335$ & $$-$0.157$ & $0.530$ & $0.346$ & $0.550$ & $0.340$ & $0.300$ & $0.258$ & $0.041$ & $1$ & $$-$0.609$ & $0.122$ & $0.644$ & $0.302$ & $$-$0.339$ & $$-$0.311$ \\ 
\% White & $0.384$ & $$-$0.609$ & $$-$0.185$ & $$-$0.011$ & $0.355$ & $0.199$ & $$-$0.247$ & $$-$0.156$ & $0.349$ & $0.500$ & $0.372$ & $0.097$ & $$-$0.483$ & $$-$0.350$ & $$-$0.261$ & $$-$0.353$ & $$-$0.185$ & $$-$0.459$ & $0.023$ & $$-$0.609$ & $1$ & $$-$0.615$ & $$-$0.962$ & $$-$0.161$ & $0.373$ & $0.374$ \\ 
\% Hispanic & $$-$0.215$ & $0.122$ & $$-$0.197$ & $$-$0.088$ & $$-$0.091$ & $$-$0.307$ & $0.259$ & $0.115$ & $$-$0.185$ & $$-$0.259$ & $$-$0.420$ & $0.230$ & $0.090$ & $$-$0.052$ & $$-$0.176$ & $0.048$ & $$-$0.197$ & $0.339$ & $$-$0.221$ & $0.122$ & $$-$0.615$ & $1$ & $0.634$ & $$-$0.014$ & $$-$0.167$ & $$-$0.091$ \\ 
Ethnic fractionalization & $$-$0.388$ & $0.644$ & $0.149$ & $0.009$ & $$-$0.336$ & $$-$0.232$ & $0.302$ & $0.217$ & $$-$0.321$ & $$-$0.505$ & $$-$0.397$ & $$-$0.032$ & $0.434$ & $0.292$ & $0.267$ & $0.318$ & $0.149$ & $0.379$ & $$-$0.082$ & $0.644$ & $$-$0.962$ & $0.634$ & $1$ & $0.153$ & $$-$0.332$ & $$-$0.343$ \\ 
Black/white segration & $$-$0.284$ & $0.302$ & $0.133$ & $$-$0.009$ & $$-$0.192$ & $$-$0.192$ & $0.341$ & $0.345$ & $$-$0.139$ & $$-$0.224$ & $$-$0.264$ & $$-$0.085$ & $0.186$ & $0.200$ & $0.276$ & $0.188$ & $0.133$ & $0.220$ & $0.081$ & $0.302$ & $$-$0.161$ & $$-$0.014$ & $0.153$ & $1$ & $$-$0.062$ & $$-$0.080$ \\ 
community.health.controlled & $0.719$ & $$-$0.339$ & $$-$0.419$ & $$-$0.294$ & $0.730$ & $0.066$ & $0.034$ & $$-$0.026$ & $0.536$ & $0.243$ & $$-$0.050$ & $0.274$ & $$-$0.626$ & $$-$0.383$ & $$-$0.253$ & $$-$0.179$ & $$-$0.419$ & $$-$0.364$ & $$-$0.392$ & $$-$0.339$ & $0.373$ & $$-$0.167$ & $$-$0.332$ & $$-$0.062$ & $1$ & $0.108$ \\ 
num\_users\_per\_map & $0.040$ & $$-$0.311$ & $$-$0.047$ & $$-$0.027$ & $0.073$ & $$-$0.094$ & $0.119$ & $0.005$ & $$-$0.036$ & $0.113$ & $$-$0.043$ & $0.195$ & $$-$0.167$ & $$-$0.230$ & $$-$0.201$ & $$-$0.310$ & $$-$0.047$ & $$-$0.103$ & $$-$0.060$ & $$-$0.311$ & $0.374$ & $$-$0.091$ & $$-$0.343$ & $$-$0.080$ & $0.108$ & $1$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 


==> figures/ngrams_top_bottom_groups.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Thu, Oct 07, 2021 - 12:26:50 PM
\begin{tabular}{@{\extracolsep{5pt}} ccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & name & ngram & n & nfactor & log\_odds\_weighted & row \\ 
\hline \\[-1.8ex] 
1 & high & county & 3471 & 2 & 11.5647285356933 & 1 \\ 
2 & high & sale & 1671 & 2 & 7.99062875031937 & 2 \\ 
3 & high & church & 2094 & 2 & 7.25212506363255 & 3 \\ 
4 & high & buy & 1374 & 2 & 7.1065169129601 & 4 \\ 
5 & high & sell & 1281 & 2 & 6.95973792821873 & 5 \\ 
6 & high & trade & 1108 & 2 & 6.12913388385456 & 6 \\ 
7 & high & area & 1319 & 2 & 5.79188052716669 & 7 \\ 
8 & high & buy sell & 868 & 2 & 5.6931568085959 & 8 \\ 
9 & high & yard & 489 & 2 & 4.45428905034406 & 9 \\ 
10 & high & for sale & 478 & 2 & 4.37426890058348 & 10 \\ 
11 & high & surrounding & 453 & 2 & 4.28490993787336 & 11 \\ 
12 & high & sell trade & 561 & 2 & 4.26579212847235 & 12 \\ 
13 & high & yard sale & 411 & 2 & 4.19517815242397 & 13 \\ 
14 & high & community & 2522 & 2 & 4.0756818678768 & 14 \\ 
15 & high & swap & 597 & 2 & 4.0403141520024 & 15 \\ 
16 & high & members & 1833 & 2 & 3.99706720773848 & 16 \\ 
17 & high & areas & 306 & 2 & 3.80923740245739 & 17 \\ 
18 & high & baptist & 659 & 2 & 3.80688060258239 & 18 \\ 
19 & high & moms & 1243 & 2 & 3.79109817532435 & 19 \\ 
20 & high & items & 303 & 2 & 3.75561398532673 & 20 \\ 
21 & high & city & 998 & 2 & 3.70642603209198 & 21 \\ 
22 & high & baptist church & 438 & 2 & 3.66015273462314 & 22 \\ 
23 & high & houston & 353 & 2 & 3.65997250000381 & 23 \\ 
24 & high & local & 485 & 2 & 3.59611892440867 & 24 \\ 
25 & high & surrounding areas & 269 & 2 & 3.50923235738261 & 25 \\ 
26 & high & garage & 316 & 2 & 3.44143378851994 & 26 \\ 
27 & high & and surrounding & 276 & 2 & 3.41137534231013 & 27 \\ 
28 & high & homeschool & 336 & 2 & 3.34669036188089 & 28 \\ 
29 & high & or & 559 & 2 & 3.31653350916676 & 29 \\ 
30 & high & san & 492 & 2 & 3.18393221140707 & 30 \\ 
\hline \\[-1.8ex] 
\end{tabular} 


==> figures/ngrams_top_mean_scores.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Thu, Oct 07, 2021 - 12:24:55 PM
\small
\begin{tabularx}{\columnwidth}{l c c @{\extracolsep{-1pt}} c @{\extracolsep{-1pt}} c} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & F1 & F2 & F3 & F4 \\ 
\hline \\[-1.8ex] 
1 & cousins & girl scout & paparazzi & homeschool \\ 
2 & clan & scout troop & auto & singles \\ 
3 & family group & troop & creations & arizona \\ 
4 & spring nail & scout & crafts & church of \\ 
5 & s family & kindergarten & custom & houston \\ 
6 & s usborne & mrs & parts & areas \\ 
7 & trip & grade & rocks & surrounding areas \\ 
8 & family & 20 21 & loving memory & county \\ 
9 & nail party & 2020 2021 & used & and surrounding \\ 
10 & extended & scouts & in loving & baptist church \\ 
11 & nail bar & pack & memory of & surrounding \\ 
12 & family page & 4 h & found & barter \\ 
13 & usborne & preschool & cars & items \\ 
14 & birthday & estates & baptist church & yardsale \\ 
15 & spring into & girl & small business & uncensored \\ 
16 & books more & neighborhood & car & buy nothing \\ 
17 & usborne books & 4th & who like & church \\ 
18 & descendants & subdivision & friends who & garage sale \\ 
19 & descendants of & neighbors & in memory & volunteers \\ 
20 & zyia party & 3rd & services & clothes \\ 
21 & s spring & hoa & sale or & yard sale \\ 
22 & virtual pampered & 2nd & memory & online yard \\ 
23 & bash & book club & or trade & pokemon \\ 
24 & chef party & committee & buy sale & garage \\ 
25 & into & 2020 & for sale & yard \\ 
26 & online pampered & neighborhood watch & jobs & local \\ 
27 & to order & 21 & avon & buy and \\ 
28 & shower & ms & businesses & fort \\ 
29 & s color & sunday & sale in & clothing \\ 
30 & april & soccer & llc & and sell \\ 
\hline \\[-1.8ex] 
\end{tabularx} 


==> figures/trust_state.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Thu, Oct 07, 2021 - 11:58:30 AM
\begin{tabular}{@{\extracolsep{5pt}} ccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & Trust in neighbors & Trust in strangers \\ 
\hline \\[-1.8ex] 
p(content gated) & $$-$0.816$ & $$-$0.813$ \\ 
p(member gated) & $$-$0.556$ & $$-$0.254$ \\ 
\hline \\[-1.8ex] 
\end{tabular} 


==> tmp_spatial.tex <==

\subsection{Spatial Regression}
Community health and FB Group indicators have strong spatial auto-correlations. Part of this auto-correlation may come from genuine spillover effects where a county with a high-social capital may have an effect on neighboring counties. Another source is measurement errors that are spatially correlated. These auto-correlations  may result in extremely conservative confidence intervals in the estimated coefficients. 

We used Moran's I to quantify the spatial auto-correlation (ref). A high value of Moran's I indicates strong auto-correlation. Unsurprisingly, a Moran's I of 0.63  confirmed the auto-correlation of the dependent variable (expected value was 0 with p<1e-14). 

We also confirmed the residuals we obtained in models 2 and 4 were also spatially auto-correlated. In model 2 ,which didn't have state fixed effects, Moran's I was 0.2716, higher than the expected value of -0.003 (p < 1e-14). In Model 4, which we used state fixed effects to account for possible regional correlations, the residuals exhibited a smaller spatial correlation (Moran's I 0.0526), but still higher than the expected value of -0.01479 (p<1e-14).

As a robustness check, we used spatial regression techniques to estimate the coefficients of the latent factors. We tried two methods to address this issue:

1) Spatial Lag Regression

A standard technique

2) Spatial Filters using Moran Eigenvectors

Using spatial eigenvectors obtained from the connectivity matrix as controls that account for auto-correlation.

In both methods, the coefficients estimated for all three factors stayed statistically significant and their magnitude did not differ from the vanilla OLS versions substantially, further confirming our results.

\comma{> spdep::impacts(m1_lag, listw = county_listw_w)
Impact measures (lag, exact):
                                            Direct      Indirect         Total
poly(log.population, 2)1             -17.638325504 -13.609387144 -31.247712648
poly(log.population, 2)2               3.190974217   2.462093325   5.653067542
poly(log.density, 2)1                 -1.964962037  -1.516126294  -3.481088331
poly(log.density, 2)2                  5.714028521   4.408832702  10.122861222
median_age                             0.222103466   0.171370692   0.393474159
percent_rural                          0.029998821   0.023146504   0.053145324
percent_black                          0.042074692   0.032464010   0.074538701
percent_non_hispanic_white            -0.036229259  -0.027953788  -0.064183046
log.median_household_income           -0.025421279  -0.019614562  -0.045035841
percent_of_housing_owner_occupied     -0.118201034  -0.091201607  -0.209402641
percent_adults_graduated_high_school   0.089711697   0.069219792   0.158931488
percent_adults_with_ba                 0.181267353   0.139862346   0.321129699
ethnic.fractionaliziation             -0.021881253  -0.016883147  -0.038764401
percent_foreign_born                   0.004434661   0.003421698   0.007856358
gini_coefficient                      -0.002192215  -0.001691470  -0.003883685
fa0.1                                  0.119103729   0.091898109   0.211001838
fa0.2                                  0.072019338   0.055568713   0.127588050
fa0.3                                  0.144650757   0.111609696   0.256260454}

\comma{> m1_esf
Call:
spmoran::esf(y = y, x = x, meig = meigB, fn = "all")

----Coefficients------------------------------
                                          Estimate          SE    t_value      p_value
(Intercept)                           -0.001984724 0.007654126 -0.2593012 7.954219e-01
poly.log.population..2.1             -14.995988894 1.838471959 -8.1567678 5.140229e-16
poly.log.population..2.2               4.465970208 0.780743349  5.7201515 1.177085e-08
poly.log.density..2.1                 -4.956934565 1.740021404 -2.8487779 4.420835e-03
poly.log.density..2.2                  4.897534527 0.874582015  5.5998574 2.353843e-08
median_age                             0.190126734 0.015756368 12.0666600 1.015279e-32
percent_rural                         -0.025035064 0.017576920 -1.4243146 1.544670e-01
percent_black                          0.134798282 0.027274498  4.9422828 8.176832e-07
percent_non_hispanic_white             0.105774952 0.030057500  3.5190868 4.399439e-04
log.median_household_income           -0.074950823 0.022239711 -3.3701348 7.615098e-04
percent_of_housing_owner_occupied     -0.119793626 0.016435496 -7.2887136 4.052516e-13
percent_adults_graduated_high_school   0.027446970 0.022201030  1.2362926 2.164537e-01
percent_adults_with_ba                 0.208057855 0.018819320 11.0555456 7.709507e-28
ethnic.fractionaliziation              0.012221489 0.022920106  0.5332213 5.939228e-01
percent_foreign_born                   0.005949632 0.019195318  0.3099522 7.566204e-01
gini_coefficient                       0.001026998 0.012344153  0.0831971 9.337008e-01
fa0.1                                  0.181149846 0.017044923 10.6277894 6.854714e-26
fa0.2                                  0.253396861 0.031628068  8.0117718 1.643683e-15
fa0.3                                  0.129753472 0.023811003  5.4493074 5.497006e-08

----Spatial effects (residuals)---------------
                      Estimate
SE                   0.4936576
Moran.I/max(Moran.I) 0.0682295

----Error statistics--------------------------
                  stat
resid_SE     0.4266441
adjR2        0.8164067
logLik   -1598.2533739
AIC       3822.5067478
BIC       5713.5697125}
